Domain-adaptive and Subgroup-specific Cascaded Temperature Regression for Out-of-distribution Calibration

Although deep neural networks yield high classification accuracy given sufficient training data, their predictions are typically overconfident or under-confident, i.e., the prediction confidences cannot truly reflect the accuracy. Post-hoc calibration tackles this problem by calibrating the prediction confidences without re-training the classification model. However, current approaches assume congruence between test and validation data distributions, limiting their applicability to out-of-distribution scenarios. To this end, we propose a novel meta-set-based cascaded temperature regression method for post-hoc calibration. Our method tailors fine-grained scaling functions to distinct test sets by simulating various domain shifts through data augmentation on the validation set. We partition each meta-set into subgroups based on predicted category and confidence level, capturing diverse uncertainties. A regression network is then trained to derive category-specific and confidence-level-specific scaling, achieving calibration across meta-sets. Extensive experimental results on MNIST, CIFAR-10, and TinyImageNet demonstrate the effectiveness of the proposed method.

==> 2.relatedwork.tex <==
\section{Related Work}
% \textbf{Calibration methods.} In machine learning, some tasks based on the deep neural network cannot truly reflect the information of the data itself due to the existence of overconfident or under-confidence prediction output \cite{nguyen2015deep,guo2017calibration}. To tackle this problem, many calibration methods have been developed. Platt scaling \cite{platt1999probabilistic, niculescu2005predicting} uses the sigmoid function to fit the output values of the model and then maps the original output values to probability values. Histogram binning \cite{gupta2021distribution} divides the confidence information into multiple bins and deals with probability changes of the confidential information in bins by setting a calibration score for each bin. Matrix scaling and Vector scaling \cite{guo2017calibration} are two extensions of Platt scaling, where the logit vector is linearly transformed before the softmax operation. Isotonic regression \cite{zadrozny2001obtaining,zadrozny2002transforming} can correct any monotonic distortion. Temperature scaling \cite{guo2017calibration} is a variant of Platt scaling and a widely used calibration algorithm. Recently, some works aim to produce overconfident predictions by designing new correction rules \cite{Wang_2021_ICCV,Gong_2021_ICCV,Ding_2021_ICCV}. Set-level, cluster-level with the nearest neighbor, and cluster-level with linear regression. \cite{Gong_2021_ICCV} proposed to use multiple calibration domains to reduce the effective distribution disparity between the target and calibration domains. 
% ~\cite{ma2021meta} utilized meta-information to enhance the calibration performance of neural networks.
% ~\cite{liu2022devil} introduced margin-based label smoothing as a calibration technique.
% ~\cite{munir2022towards} focused on improving calibration performance in the context of object detection tasks when faced with variations in domains.
% The above methods can perform well under ID scenarios but are not suitable for OOD scenarios. While the main theme of the paper is solving the task of post-hoc uncertainty calibration under OOD scenarios.
\textbf{Calibration methods.}In machine learning, deep neural networks suffer from overconfident or under-confident predictions that fail to accurately reflect the inherent data information~\cite{nguyen2015deep,guo2017calibration}. To counter this issue, various calibration methods have emerged. Platt scaling~\cite{platt1999probabilistic,niculescu2005predicting} employs a sigmoid function to align model outputs with probability values. 
Histogram binning~\cite{gupta2021distribution} segregates confidence data into bins, assigning calibration scores to each. 
Matrix and Vector scaling~\cite{guo2017calibration} extend Platt scaling through logit vector transformation pre-softmax. 
Isotonic regression \cite{zadrozny2001obtaining,zadrozny2002transforming} corrects monotonic distortions. Temperature scaling~\cite{guo2017calibration}, a Platt scaling variant, is widely used. Some works design new correction rules for overconfident predictions~\cite{Wang_2021_ICCV,Gong_2021_ICCV}, employing various techniques like set-level and cluster-level corrections.
Recent approaches address calibration enhancement. ~\cite{ma2021meta} leverages meta-information, while~\cite{liu2022devil} introduces margin-based label smoothing.
The above methods can perform well under ID scenarios but are not suitable for OOD scenarios. While the main theme of the paper is solving the task of post-hoc calibration under OOD scenarios.%uncertainty 

% \textbf{Calibration under OOD.} Little research has been conducted in the uncertainty calibration under OOD scenarios~\cite{liang2017enhancing,jiang2018trust,papernot2018deep,tomani2021post,yu2022robust}. Among those approaches, ~\cite{jiang2018trust,papernot2018deep} draw attention to deriving trust score and other measures for out-of-distribution detection to detect truly OOD instances, which is useful for understanding the prediction performance of a model. 
% ~\cite{liang2017enhancing,tomani2021post} are based on the principle of adding perturbations to the instances in the validation set before performing the post-hoc calibration step, which can separate the softmax score distributions between ID and OOD instances and allowing for more effective detection. Differently, we aim to realize the calibration of category-wise confidence and confidence-level-wise confidence by utilizing the meta-set at all stages of domain drift.
\textbf{Calibration under OOD.} Limited research addresses uncertainty calibration in OOD scenarios ~\cite{liang2017enhancing,jiang2018trust,papernot2018deep,tomani2021post}. Among those approaches,~\cite{jiang2018trust,papernot2018deep} draw attention to deriving trust score and other measures for out-of-distribution detection to detect truly OOD instances, enhancing understanding of model prediction performance.
~\cite{liang2017enhancing,tomani2021post} introduce perturbations to the validation set instances before calibration, effectively distinguishing softmax score distributions between ID and OOD instances for better detection. Differently, we aim to realize the calibration of category-wise confidence and confidence-level-wise confidence by utilizing the meta-set at all stages of domain drift.
